A Document Skew Detection Method Using Fast Hough Transform

The majority of document image analysis systems use a document skew detection algorithm to simplify all its further processing stages. A huge amount of such algorithms based on Hough transform (HT) analysis has already been proposed. Despite this, we managed to find only one work where the Fast Hough Transform (FHT) usage was suggested to solve the indicated problem. Unfortunately, no study of that method was provided. In this work, we propose and study a skew detection algorithm for the document images which relies on FHT analysis. To measure this algorithm quality we use the dataset from the problem oriented DISEC'13 contest and its evaluation methodology. Obtained values for AED, TOP80, and CE criteria are equal to 0.086, 0.056, 68.80 respectively.

==> by_image.tex <==
\begin{tabular}{lrrrrrr}
\toprule
{} &    AED &  TOP80 &   CE &    MAX &    MIN &  RANGE \\
\midrule
74 &  0.279 &  0.249 &  0.0 &  0.417 &  0.125 &  0.292 \\
18 &  0.260 &  0.235 &  0.0 &  0.406 &  0.124 &  0.282 \\
20 &  0.246 &  0.222 &  0.0 &  0.355 &  0.109 &  0.246 \\
68 &  0.307 &  0.299 &  0.0 &  0.340 &  0.266 &  0.074 \\
61 &  0.256 &  0.245 &  0.0 &  0.315 &  0.211 &  0.104 \\
99 &  0.237 &  0.225 &  0.0 &  0.308 &  0.182 &  0.126 \\
84 &  0.253 &  0.244 &  0.0 &  0.305 &  0.202 &  0.103 \\
40 &  0.243 &  0.232 &  0.0 &  0.289 &  0.212 &  0.077 \\
65 &  0.228 &  0.220 &  0.0 &  0.265 &  0.183 &  0.082 \\
35 &  0.229 &  0.222 &  0.0 &  0.258 &  0.188 &  0.070 \\
\bottomrule
\caption{group by image}
\label{tbl:group_by_image}
\end{tabular}

==> groups2.tex <==

% How to build this table: python disec13_stat.py -r <run name> -a

Table with residuals grouped by angle is presented in \ref{tbl:group_by_angle}.


\begin{table}[ht]
\centering
\begin{tabular}{lrrrrrrr}
angle\_gt &  COUNT &    AED &  TOP80 &      CE &    MAX &    MIN &  RANGE \\
(-15.0, -14.0] &     54 &  0.093 &  0.063 &  66.667 &  0.339 &  0.002 &  0.337 \\
(-14.0, -13.0] &     55 &  0.084 &  0.053 &  72.727 &  0.315 &  0.000 &  0.315 \\
(-13.0, -12.0] &     47 &  0.091 &  0.064 &  59.574 &  0.417 &  0.003 &  0.414 \\
(-12.0, -11.0] &     42 &  0.079 &  0.050 &  66.667 &  0.235 &  0.002 &  0.233 \\
(-11.0, -10.0] &     53 &  0.081 &  0.053 &  66.038 &  0.340 &  0.001 &  0.339 \\
(-10.0, -9.0]  &     54 &  0.102 &  0.072 &  61.111 &  0.331 &  0.000 &  0.331 \\
(-9.0, -8.0]   &     44 &  0.089 &  0.058 &  65.909 &  0.417 &  0.002 &  0.415 \\
(-8.0, -7.0]   &     52 &  0.100 &  0.067 &  53.846 &  0.446 &  0.006 &  0.440 \\
(-7.0, -6.0]   &     55 &  0.085 &  0.056 &  70.909 &  0.308 &  0.004 &  0.304 \\
(-6.0, -5.0]   &     46 &  0.074 &  0.049 &  71.739 &  0.278 &  0.001 &  0.277 \\
(-5.0, -4.0]   &     54 &  0.093 &  0.059 &  61.111 &  0.547 &  0.003 &  0.544 \\
(-4.0, -3.0]   &     49 &  0.064 &  0.041 &  79.592 &  0.258 &  0.000 &  0.258 \\
(-3.0, -2.0]   &     53 &  0.094 &  0.058 &  67.925 &  0.500 &  0.002 &  0.498 \\
(-2.0, -1.0]   &     48 &  0.090 &  0.059 &  68.750 &  0.314 &  0.001 &  0.313 \\
(-1.0, 0.0]    &     60 &  0.079 &  0.052 &  68.333 &  0.253 &  0.005 &  0.248 \\
(0.0, 1.0]     &     38 &  0.088 &  0.058 &  63.158 &  0.308 &  0.007 &  0.301 \\
(1.0, 2.0]     &     58 &  0.078 &  0.053 &  70.690 &  0.253 &  0.000 &  0.253 \\
(2.0, 3.0]     &     59 &  0.084 &  0.052 &  66.102 &  0.272 &  0.001 &  0.271 \\
(3.0, 4.0]     &     57 &  0.088 &  0.054 &  66.667 &  0.406 &  0.004 &  0.402 \\
(4.0, 5.0]     &     56 &  0.091 &  0.057 &  64.286 &  0.319 &  0.003 &  0.316 \\
(5.0, 6.0]     &     57 &  0.077 &  0.048 &  68.421 &  0.305 &  0.002 &  0.303 \\
(6.0, 7.0]     &     50 &  0.088 &  0.060 &  60.000 &  0.289 &  0.003 &  0.286 \\
(7.0, 8.0]     &     43 &  0.073 &  0.047 &  81.395 &  0.270 &  0.002 &  0.268 \\
(8.0, 9.0]     &     54 &  0.082 &  0.052 &  66.667 &  0.376 &  0.001 &  0.375 \\
(9.0, 10.0]    &     57 &  0.095 &  0.064 &  63.158 &  0.304 &  0.009 &  0.295 \\
(10.0, 11.0]   &     55 &  0.079 &  0.051 &  69.091 &  0.286 &  0.001 &  0.285 \\
(11.0, 12.0]   &     49 &  0.095 &  0.062 &  59.184 &  0.355 &  0.001 &  0.354 \\
(12.0, 13.0]   &     46 &  0.081 &  0.047 &  71.739 &  0.329 &  0.002 &  0.327 \\
(13.0, 14.0]   &     46 &  0.093 &  0.062 &  65.217 &  0.291 &  0.003 &  0.288 \\
(14.0, 15.0]   &     59 &  0.079 &  0.049 &  69.492 &  0.266 &  0.001 &  0.265 \\
\end{tabular}
\caption{group by angle}
\label{tbl:group_by_angle}
\end{table}
